A quasilinear complexity algorithm for the numerical simulation of scattering from a two-dimensional radially symmetric potential

Standard solvers for the variable coefficient Helmholtz equation in two spatial dimensions have running times which grow quadratically with the wavenumber $k$. Here, we describe a solver which applies only when the scattering potential is radially symmetric but whose running time is $\mathcal{O}\left(k \log(k) \right)$ in typical cases. We also present the results of numerical experiments demonstrating the properties of our solver, the code for which is publicly available.

==> plane_table.tex <==
\begin{tabular}{crccc}
\toprule
 \addlinespace[.25em]
$k$                                &$m$                                &Maximum absolute                   &Precomp time                       &Solve time                        \\
                                   &                                   &error                              &(in seconds)                       &(in seconds)                       \\
\midrule
 \addlinespace[.25em]
$2^{4}$ &  100 & 1.72\e{-11} & 1.01\e{-01} & 1.35\e{-04}  \\
 \addlinespace[.125em]
$2^{5}$ &  201 & 4.23\e{-11} & 1.91\e{-01} & 2.20\e{-04}  \\
 \addlinespace[.125em]
$2^{6}$ &  402 & 1.12\e{-10} & 3.68\e{-01} & 4.80\e{-04}  \\
 \addlinespace[.125em]
$2^{7}$ &  804 & 3.10\e{-10} & 7.22\e{-01} & 6.19\e{-03}  \\
 \addlinespace[.125em]
$2^{8}$ & 1608 & 8.73\e{-10} & 1.43\e{+00}  & 2.41\e{-02}  \\
 \addlinespace[.125em]
 \addlinespace[.25em]
\bottomrule
\end{tabular}

